A Block-wise, Asynchronous and Distributed ADMM Algorithm for General Form Consensus Optimization

Many machine learning models, including those with non-smooth regularizers, can be formulated as consensus optimization problems, which can be solved by the alternating direction method of multipliers (ADMM). Many recent efforts have been made to develop asynchronous distributed ADMM to handle large amounts of training data. However, all existing asynchronous distributed ADMM methods are based on full model updates and require locking all global model parameters to handle concurrency, which essentially serializes the updates from different workers. In this paper, we present a novel block-wise, asynchronous and distributed ADMM algorithm, which allows different blocks of model parameters to be updated in parallel. The lock-free block-wise algorithm may greatly speedup sparse optimization problems, a common scenario in reality, in which most model updates only modify a subset of all decision variables. We theoretically prove the convergence of our proposed algorithm to stationary points for non-convex general form consensus problems with possibly non-smooth regularizers. We implement the proposed ADMM algorithm on the Parameter Server framework and demonstrate its convergence and near-linear speedup performance as the number of workers increases.

==> src/approx.tex <==
%!TEX root = ../main.tex

\section{Approximate Update for Communication Efficiency}
\label{sec:approx}

In this section, we will discuss some techniques in practice to lower the communication cost. As reported in the literature, e.g., \cite{li2014communication}, bandwidth in datacenters is often 10-100 times smaller than memory bandwidth, which limits to support a large scale cluster with more than 1000 workers and servers.

\subsection{Pushing Changes, not Variables}
We firstly try to lower the parameters transmitted from workers to servers. In SGD-based methods, workers will transmit gradients, which are decreasing towards zero along with iterations. Therefore, the communication cost can be lower when the magnitude of gradients are small. Unlike SGD-based methods, however, workers in Algorithm~\ref{alg:admm-worker} transmits an aggregation of its local variable $x_{i,j}^{t+1}$ and its dual variable $y_{i,j}^{t+1}$, which are changed slightly but may still have significant magnitudes. Sending the change in the local variables rather than themselves can also ensure that, when updating the global variables, a fast worker node does not bias the global variable $z_j$ towards its own $x_{i,j}$ when performing multiple updates in short period of epochs.

Particularly, we set another variable $s_j^{t+1}$ to denote the sum of all received updates from workers as:
\begin{equation}
	s_j^{t+1} := \sum_{i \in \mathcal{N}(j)} \hat{w}_{i,j}^{t+1}.
\end{equation}
Then, we can rewrite the update step \eqref{eq:update_z} as
\begin{equation}
	z_j^{t+1} = \prox[\mu]{h}\left( \frac{\gamma z_j^t + s_j^{t+1}}{\sum_{i \in \mathcal{N}(j)}\rho_{i,j}}  \right).
	\label{eq:update_z2}
\end{equation}
Let $\Delta x_{i,j}^{t+1}$ denote $x_{i,j}^{t+1}-x_{i,j}^t$ and $\Delta y_{i,j}^{t+1}$ denote $y_{i,j}^{t+1}-y_{i,j}^t$. By simple algebra we can easily have
\begin{equation}
	s_j^{t+1} = s_j^{t} + \rho_{i,j} \Delta x_{i,j}^{t+1} + \Delta y_{i,j}^{t+1}.
	\label{eq:update_s}
\end{equation}
To rewrite Algorithm~\ref{alg:admm-worker}, we replace Step 7 by pushing $\rho_{i,j}\Delta x_{i,j} + \Delta y_{i,j}$ to server $j$. To rewrite Algorithm~\ref{alg:admm-server}, server $j$ receives $\rho_{i,j} \Delta x_{i,j}^{t+1} + \Delta y_{i,j}^{t+1}$ and update $s_j^{t+1}$ according to \eqref{eq:update_s} and further update $z_j^{t+1}$ according to \eqref{eq:update_z2}.

However, we should note that this scheme may lead to divergence without proper initialization. Note that $s_j^{t+1}$ can be correctly calculated using \eqref{eq:update_s}, provided that $s_j^{0}$ equals with the sum of $\rho_{i,j}x_{i,j}^0 + y_{i,j}^0$ for all $i \in \mathcal{N}(j)$. One way is to initialize all variables, including $x_{i,j}$, $y_{i,j}$, $s_j$ and $z_j$, as $0$. Another way is to set up a synchronization update in initialization. Since this is the only one synchronization step in the algorithm, the time consumption can be tolerated, and we can utilize such step to test link communication.

\subsection{Significance Filters}
We can further reduce the communication overhead by ensuring the local copy $x_{i,j}$ is \emph{approximately correct}, which eliminates insignificant and unnecessary communication between workers and servers. Such scheme is widely adopted in SGD-based distributed machine learning systems, i.e., parameter server \cite{li2014scaling} and Gaia \cite{hsieh17gaia}. As reported in \cite{hsieh17gaia}, nearly 95\% updates are causing 1\% change on the parameter values and we can conclude that the vast majority of changes are quite insignificant.

\begin{thm}
	Suppose that Assumption~\ref{asmp:lipschitz}-\ref{asmp:delay} hold. Assume that we apply a significant filter on pushing values with threshold $\delta_{i,j}^{t} = O(t^{-1})$ and penalty parameters $\rho_{i,j}$ and $\gamma$ are chosen such that
	{\small
	\begin{align}
	\infty & > L(\mathbf{X}^0, \mathbf{z}^0, \mathbf{Y}^0) - \underline{f} \geq 0 \\
	\alpha'_{i,j} &:= \frac{\rho_{i,j}+\gamma-\delta_{i,j}^t}{2} - \left(\frac{7L_{i,j}}{2\rho_{i,j}^2} + \frac{1}{\rho_{i,j}}\right) L_{i,j}^2(T_{i,j}+1)^2 - \frac{T_{i,j}^2}{2}  \nonumber \\
	& > 0, \forall t>0, \\
	\beta'_{i,j} &:= \frac{\rho_{i,j}}{4} - 3L_{i,j} > 0, \quad (i,j) \in \mathcal{E}.
	\end{align}
	}
	Then Algorithm~\ref{alg:admm-worker}-\ref{alg:admm-server} can converge in expectation to stationary points satisfying KKT conditions.
	\label{thm:approx}
\end{thm}
The proof of this Theorem is similar with that of Theorem~\ref{thm:convergence}. The high level idea of this theorem is that, the update for $\mathbf{z}^{t+1}$ is \emph{``contaminated'' by quantization noise}. In other words, if we apply a significance filter with the threshold of $\delta_{i,j}^t$ on $w_{i,j}^t:=\rho_{i,j}\Delta x_{i,j}^t + \Delta y_{i,j}^t$, we can regard the newly pushed value $\tilde{w}_{i,j}^{t} = w_{i,j}^t + \epsilon_{i,j}^t$, where $\epsilon_{i,j}^t$ is a random noise with the magnitude of $\delta_{i,j}^t$.

Similarly, from the strongly convexity of $L(\mathbf{X}, \mathbf{z}, \mathbf{Y})$ w.r.t. $\mathbf{z}$, we have
\begin{align}
& L(\mathbf{X}^t, \mathbf{z}^{t+1}, \mathbf{Y}^t) - L(\mathbf{X}^t, \mathbf{z}^{t}, \mathbf{Y}^t) \\
&\leq \innerprod{\mathbf{s}+\epsilon_{i,j}^{t+1}, \mathbf{z}^t - \mathbf{z}^{t+1}} \nonumber \\
& - \sum_{i=1}^N\sum_{j \in \mathcal{N}(i)} \left( \frac{\rho_j}{2} \norm{z_j^{t+1} - z_j^{t}}^2 + \frac{\gamma}{2} \norm{z_j^{t+1} - z_j^{t}}\right)\\
&= \sum_{(i,j) \in \mathcal{E}} \epsilon_{i,j}^{t+1}({z}_j^t - {z}_j^{t+1})-\frac{\rho_{i,j}+\gamma}{2} \norm{z_j^{t+1} - z_j^{t}}^2,
\label{eq:noisy-1}
\end{align}
where $\mathbf{s} \in \partial h(\mathbf{z}^{t+1})$. By take the expectation of the above equation, we have
\begin{eqnarray}
&& \mathbf{E}[L(\mathbf{X}^t, \mathbf{z}^{t+1}, \mathbf{Y}^t) - L(\mathbf{X}^t, \mathbf{z}^{t}, \mathbf{Y}^t)] \nonumber \\
&\leq& \sum_{(i,j) \in \mathcal{E}} \delta_{i,j}^{t+1}\norm{{z}_j^t - {z}_j^{t+1}}-\frac{\rho_{i,j}+\gamma}{2} \norm{z_j^{t+1} - z_j^{t}}^2 \\
&\leq& -\sum_{(i,j) \in \mathcal{E}}\frac{\delta_{i,j}^{t+1}-(\rho_{i,j}+\gamma)}{2} \norm{z_j^{t+1} - z_j^{t}}^2.
\label{eq:noisy-2}
\end{eqnarray}
The equation \eqref{eq:diff1-2} and \eqref{eq:diff1-3} can be similarly adopted. Combining \eqref{eq:diff1-2}, \eqref{eq:diff1-3} and \eqref{eq:noisy-2}, we have similar result on like \ref{eq:iteration_L} and finally proves Theorem~\ref{thm:approx}.
% The proof is shown in Appendix. 
When approaching to a stationary point, the changes $\Delta x_{i,j}^{t}$ will vanish. Therefore, like SGD and SPGD based methods, inexact changes obtained by delayed and inexact global model could be good approximation of the ground true one. One difference here is that the threshold $\delta_{i,j}$ can be set as a constant, while in SGD or SPGD based methods, the threshold should decrease to ensure convergence. For example, in Gaia, the threshold will be decreased as $O(1/\sqrt{t})$ \cite{hsieh17gaia}.

==> src/related.tex <==
%!TEX root = ../main.tex

\section{Related Work}
\label{sec:related}

Distributed ADMM has been widely discussed in the literature. The original distributed ADMM can be found in \cite{boyd2011distributed}, which is a synchronous algorithm with fully updates. In this work, Eq.~\eqref{eq:admm-basic-1} is performed on the master node and Eq.~\eqref{eq:admm-basic-2}-\eqref{eq:admm-basic-3} are performed on each worker node $i$. It can be shown to converge to a Karush-Kuhn-Tucker (KKT) point event for both convex and non-convex problems \cite{hong2016convergence}.

Extending consensus ADMM to the asynchronous setting has been discussed in recent years. In \cite{zhang2014asynchronous}, they consider a asynchronous consensus ADMM with assumption on bounded delay, but only convex cases are analyzed. References \cite{chang2016asynchronous1,chang2016asynchronous2} propose a asynchronous ADMM algorithm with analysis on both convex and nonconvex cases. However, they require each worker solve a subproblem exactly and it might be time costly in some cases. Reference \cite{hong2017distributed} proposes another asynchronous algorithm that each worker only calculates gradients and updates of all $\mathbf{x}_i,\mathbf{y}_i$ and $\mathbf{z}$ are done on the server side, which can consume a lot of memory in a large cluster. References \cite{wei20131,mota2013d} consider asynchronous ADMM for decentralized networks. In particular, reference \cite{wei20131} assumes that communication links between nodes can fail randomly and provides convergence analysis in a probability-one sense.

To our best knowledge, existing asynchronous ADMM algorithms do not support blockwise updates and this paper tries to make the first attempt to study blockwise updates in asynchronous settings. 
Existing blockwise updates are considered in stochastic gradient descent \cite{lian2015asynchronous}, proximal gradient descent \cite{li2014communication}, block or stochastic coordinate descent (BCD or SCD) \cite{liu2015asynchronous} and a recently proposed block successive upper bound minimization method (BSUM) \cite{razaviyayn2013unified}. For SGD type algorithms, their convergence rate can be low. For BCD type algorithms, it is preferred that datasets are partitioned by features, which limits its applications.

